The Music Annotation Pattern

The annotation of music content is a complex process to represent due to its inherent multifaceted, subjectivity, and interdisciplinary nature. Numerous systems and conventions for annotating music have been developed as independent standards over the past decades. Little has been done to make them interoperable, which jeopardises cross-corpora studies as it requires users to familiarise with a multitude of conventions. Most of these systems lack the semantic expressiveness needed to represent the complexity of the musical language and cannot model multi-modal annotations originating from audio and symbolic sources. In this article, we introduce the Music Annotation Pattern, an Ontology Design Pattern (ODP) to homogenise different annotation systems and to represent several types of musical objects (e.g. chords, patterns, structures). This ODP preserves the semantics of the object's content at different levels and temporal granularity. Moreover, our ODP accounts for multi-modality upfront, to describe annotations derived from different sources, and it is the first to enable the integration of music datasets at a large scale.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> sections/3_JAMS_ontology.tex <==
\begin{document}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% NOT INCLUDED IN THE CURRENT VERSION OF THE PAPER 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As mentioned in the previous section, JAMS \cite{humphrey2014jams} is the de-facto standard for music annotation in the field of Music Information Retrieval.
A sample JAMS file can be found in Listing \ref{list:jams-1} and \ref{list:jams-2}.


\noindent\begin{minipage}[t]{.45\textwidth}
\begin{lstlisting}[captionpos=b, numbers=left,
    numberstyle=\tiny, caption={Excerpt of the three first chords in a JAMS file annotating Queen's Bohemian Rhapsody.}, label={lst:jams-example-1},
    basicstyle=\scriptsize\ttfamily,frame=single,
    escapeinside={+}{+}, firstnumber=auto, showstringspaces=false, belowcaptionskip=0em]
{
    "sandbox": {}, 
    "annotations": [
      {
        "data": [
          {
            "duration": 0.459, 
            "confidence": 1.0, 
            "value": "N", 
            "time": 0.0
          }, 
          {
            "duration": 3.663, 
            "confidence": 1.0, 
            "value": "Bb:maj6", 
            "time": 0.459
          }, 
          {
            "duration": 0.789, 
            "confidence": 1.0, 
            "value": "C:7", 
            "time": 4.122
          }, 
          ...
          ], 
\end{lstlisting}
\label{list:jams-1}
\end{minipage}\hfill
\begin{minipage}[t]{.45\textwidth}
\begin{lstlisting}[captionpos=b, numbers=left,
    numberstyle=\tiny, caption={Annotation and file metadata in a JAMS file annotating Queen's Bohemian Rhapsody.}, label={lst:jams-example-2},
    basicstyle=\scriptsize\ttfamily,frame=single,
    escapeinside={+}{+}, firstnumber=auto, showstringspaces=false, belowcaptionskip=0em]
        "annotation_metadata": {
          "annotation_tools": "", 
          "curator": {
            "name": "Matthias Mauch", 
            "email": "m.mauch@qmul.ac.uk"
          }, 
          "annotator": {}, 
          "version": 1.0, 
          "corpus": "Isophonics", 
          "annotation_rules": "", 
          "validation": "", 
          "data_source": ""
        }, 
        "namespace": "chord", 
        "sandbox": {}
      }, ... ],
      "file_metadata": {
        "jams_version": "0.2.0", 
        "title": "01 Bohemian Rhapsody", 
        "identifiers": {}, 
        "release": "", 
        "duration": 358.293, 
        "artist": "Queen"
    }
}
\end{lstlisting}
\label{list:jams-2}
\end{minipage}




However, JAMS present several semantic limitations, which affect significantly the expressiveness of the standard.
For example, JAMS does not allow to define whether the contained annotations come from a signal representation rather than a symbolic representation. 
This also leads to a discrepancy between the content of the annotations themselves: audio-based annotations express temporal information in real time (usually in seconds), whereas symbolic temporal annotations are generally expressed in beats and measures. 
At the same time, it is not possible to distinguish between different types of annotations contained in the metadata. For instance, it is not possible to define whether the artist described in the JAMS is the composer or the performer of the track. 
As a result, it is not even possible to define the relationship between the artist and the song annotated in the JAMS file.

However, it is possible to add this information within the JAMS file, expanding it thanks to the native possibility of extending both its namespaces and adding data within fields called sandboxes. However, it is not possible to define the type of relationship between the different fields and consequently how they interact with each other. 

These limitations led us to the definition of the JAMS ontology, a model for semantically enriching musical annotations that can at the same time be standardised according to a common model. 
The ontology is already available online at the following URI:

\begin{center}
\texttt{\url{https://w3id.org/polifonia/ontology/jams/}}
\end{center}

It is important to clarify that the same terms used in the JAMS documentation\footnote{Official JAMS documentation: \url{https://jams.readthedocs.io/en/stable/}} have been reused in the modelling of this ontology.
In particular, the following terms are used:
\begin{itemize}
    \item \textbf{Annotation: } an annotation is defined as a group of \texttt{Observations} (see below) that share certain elements, such as the method used for the annotation and the type of annotation contained (e.g. chords, notes, patterns);
    \item \textbf{Observation: } an observation is defined as the content of the annotation, and includes all elements that characterise the observation. For example, in the case of an annotation containing chords, each observation corresponds to a chord, but also specifies, in addition to the chord value, the temporal information and the confidence of the annotated observation. 
\end{itemize}

In this first iteration, we focused only on the annotations of music chords, not considering all other types of annotations that the JAMS file may contain. 
However, we propose the \emph{Music Annotation Pattern}, an ODP that serves as a reusable building block for modelling any type of music annotation, whether annotated from audio or music score. 

\subsection{Ontology Modelling and Testing}

The JAMS ontology was modelled and tested following the approach named eXtreme design \cite{presutti2009xd}.
Competency questions (CQs) were then defined in order to collect the necessary requirements for modelling the ontology and its subsequent testing.  
The identified competency questions are listed in Table \ref{tab:cqs}.

\begin{table}[bp]
\begin{tabular}{ll}

\hline
ID   & Competency question                                    \\
\hline
CQ1  & What is the type of the annotation for a track?        \\
CQ2  & Who is the composer of the track?                      \\
CQ3  & Who is the performer of the track?                     \\
CQ4  & How was the annotation made?                           \\
CQ5  & What is the length of the annotation?                  \\
CQ6  & Where does the annotation start?                       \\
CQ7  & Which are the observation for each annotation?         \\
CQ8  & For a specific observation, what is its starting time? \\
CQ9  & For a specific observation, what is its duration?      \\
CQ10 & What is the key of the annotation?                     \\
CQ11 & For a specific observation, what is its value (chord)? \\
\hline
\end{tabular}
\caption{Competency questions (CQs) for the JAMS Ontology.}
\label{tab:cqs}
\end{table}

Figure \ref{fig:annotation-module} shows the first part of the ontology, describing an \emph{annotation} and its attributes.

Classes and properties from the \emph{Polifonia Ontology Network (PON)} are reused for the definition of artist metadata. In particular, classes and properties from the PON modules \emph{core}, \emph{muiscal feature}, \emph{musical composition} and \emph{musical performance} are reused. 
Through the use of these modules, it is possible to define a musical composition \texttt{mc:MusicalComposition} and the score on which it is based \texttt{mf:Score}, and the recording, intended as the realisation of a musical composition \texttt{mf:Recording}. 
Each of these classes is linked to a \texttt{core:Agent} class, which defines the composer or the performer, respectively.

\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth]{images/jams-ontology.png}
    \caption{Fragment of the JAMS ontology describing JAMS files and their provenance, musical objects and JAMS annotations. We use the Graffoo notation%\footnote{\url{https://essepuntato.it/graffoo/}}
    : yellow boxes are classes, blue/green arrows are object/datatype properties, purple circles are individuals, green polygons are datatypes.}
    \label{fig:annotation-module}
\end{figure*}

The central class of the ontology is the \texttt{jams:JAMSAnnotation}, which corresponds to an annotation of a specific track. The annotation then has a certain duration \texttt{jams:hasValidityDuration} and an annotator \texttt{jams:Annotator}.
The annotator may be of different types, defined by the class \texttt{jams:AnnotatorType}.

The Provenance Ontology \cite{lebo2013prov} was also reused to define the provenance of the \texttt{jams:JAMSAnnotation} and link it to the \texttt{jams:JAMSFile}, \texttt{jams:JAMSAnnotation} and \texttt{mf:Corpus} from which the annotation is derived. 

The \texttt{jams:JAMSAnnotation} has two subclasses, namely \texttt{jams:JAMSScoreAnnotation} and \texttt{jams:JAMSAudioAnnotation}.
The former refers to annotations of an audio type, while the latter is used to describe annotations derived from a symbolic representation. 
The main difference between the two lies in the way the time indications of the annotation are expressed. For audio-based annotations, time indications are expressed in seconds by means of the DataType Property \texttt{jams:hasValdityStartingTime}, whereas score-based annotations are linked to the class \texttt{jams:MetricalTime}.

The \texttt{jams:MetricalTime} class describes precisely the symbolic time as expressed in symbolic notations by means of the DataType Properties \texttt{jams:hasMeasure} and \texttt{jams:hasBeat}. 

In turn, each \texttt{jams:JAMSAnnotation}, whether score or audio, contains a series of \texttt{jams:JAMSObservation}. 
The part of the ontology describing the JAMS observations is shown in Figure \ref{fig:observation-module}.


\begin{figure*}[tp]
    \centering
    \includegraphics[width=\textwidth]{images/annotations.png}
    \caption{Fragment of the JAMS ontology describing JAMS files and their provenance, musical objects and JAMS annotations. We use the Graffoo notation: yellow boxes are classes, blue/green arrows are object/datatype properties, purple circles are individuals, green polygons are datatypes.}
    \label{fig:observation-module}
\end{figure*}


\end{document}
